On the Impact of Control Signaling in RIS-Empowered Wireless Communications

The research on Reconfigurable Intelligent Surfaces (RISs) has dominantly been focused on physical-layer aspects and analyses of the achievable adaptation of the wireless propagation environment. Compared to that, questions related to system-level integration of RISs have received less attention. We address this research gap by analyzing the necessary control/signaling operations that are necessary to integrate RIS as a new type of wireless infrastructure element. We build a general model for evaluating the impact of control operations along two dimensions: i) the allocated bandwidth of the control channels (in-band and out-of-band), and ii) the rate selection for the data channel (multiplexing or diversity). Specifically, the second dimension results in two generic transmission schemes, one based on channel estimation and the subsequent optimization of the RIS, while the other is based on sweeping through predefined RIS phase configurations. We analyze the communication performance in multiple setups built along these two dimensions. While necessarily simplified, our analysis reveals the basic trade-offs in RIS-assisted communication and the associated control operations. The main contribution of the paper is a methodology for systematic evaluation of the control overhead in RIS-aided networks, regardless of the specific control schemes used.

==> acronyms.tex <==
%%%%%%%%% List of acronyms %%%%%%%%%%%
\newacronym{3d}{3D}{three dimensional}
\newacronym{aoa}{AoA}{angle of arrival}
\newacronym{aod}{AoD}{angle of departure}
\newacronym{ap}{AP}{access point}
\newacronym{awgn}{AWGN}{additive white gaussian noise}
\newacronym{b5g}{B5G}{Beyond-5G}
\newacronym{BSW}{BSW}{beam sweeping}
\newacronym{bsw}{CB-BSW}{codebook-based beam sweeping}
\newacronym[plural=BSs, firstplural=base stations (BSs)]{bs}{BS}{base station}
\newacronym{ctrl}{ctrl}{control}
\newacronym{cc}{CC}{control channel}
\newacronym{cdf}{CDF}{cumulative density function}
\newacronym{ce}{CE}{channel estimation}
\newacronym{oce}{OPT-CE}{optimization based on channel estimation}
\newacronym{obcc}{OB-CC}{out-of--band \gls{cc}} 
\newacronym{csi}{CSI}{channel state information}
\newacronym{dc}{DC}{data channel}
\newacronym{dl}{DL}{downlink}
\newacronym{dft}{DFT}{discrete Fourier transform}
\newacronym{doa}{DoA}{direction-of-arrival}
\newacronym{emf}{EMF}{electromagnetic field}
\newacronym{em}{EM}{electromagnetic}
\newacronym{fp}{FP}{fractional program}
\newacronym[plural=HRISs, firstplural=Hybrid Reconfigurable Intelligent Surfaces (HRISs)]{hris}{HRIS}{hybrid reconfigurable intelligent surface}
\newacronym{ibcc}{IB-CC}{in-band \gls{cc}}
\newacronym{ibno}{IB-no}{IB-no}
\newacronym{ibwf}{IB-wf}{IB-wf}
\newacronym{ios}{IoS}{Internet-of-Surfaces}
\newacronym{iot}{IoT}{Internet-of-Things}
\newacronym{iid}{i.i.d.}{independently identically distributed}
\newacronym[plural=KPIs, firstplural=key performance indicators (KPIs)]{kpi}{KPI}{key performance indicator}
\newacronym{lf}{LF}{low frequency}
\newacronym{los}{LoS}{line-of-sight}
\newacronym{mac}{MAC}{medium access control}
\newacronym{mcs}{MCS}{modulation and coding scheme}
\newacronym{mimo}{MIMO}{multiple-input multiple-output}
\newacronym{miso}{MISO}{multiple-input single-output}
\newacronym{ml}{ML}{machine learning}
\newacronym{mmse}{MMSE}{minimum mean squared error}
\newacronym{mrt}{MRT}{maximum-ratio transmission}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{nlos}{NLoS}{non-line-of-sight}
\newacronym{ofdm}{OFDM}{orthogonal frequency-division multiplexing}
\newacronym{pdf}{pdf}{probability distribution function}
\newacronym{pla}{PLA}{planar linear array}
\newacronym{pap}{P\&P}{plug-and-play}
\newacronym{phy}{PHY}{physical-layer}
\newacronym{ppp}{PPP}{Poisson point process}
\newacronym[plural=RISs, firstplural=Reconfigurable intelligent surfaces (RISs)]{ris}{RIS}{reconfigurable intelligent surface}
\newacronym{risc}{RISC}{\gls{ris} controller}
\newacronym{rf}{RF}{radio frequency}
\newacronym{rmse}{RMSE}{root-mean-square error}
\newacronym{rss}{RSS}{received signal strength}
\newacronym{se}{SE}{spectral efficiency}
\newacronym{sdp}{SDP}{semidefinite programming}
\newacronym{sdr}{SDR}{semidefinite relaxation}
\newacronym{sinr}{SINR}{signal-to-interference-plus-noise ratio}
\newacronym{smse}{SMSE}{sum mean squared error}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{soa}{SoA}{state-of-the-art}
\newacronym{sre}{SRE}{smart radio environment}
\newacronym{toa}{ToA}{time-of-arrival}
\newacronym{tdd}{TDD}{time division multiplex}
\newacronym{tti}{TTI}{transmission time interval}
\newacronym[plural=UEs, firstplural=users equipment (UEs)]{ue}{UE}{user equipment}
\newacronym{ul}{UL}{uplink}
\newacronym{ula}{ULA}{uniform linear array}
\newacronym{urllc}{URLLC}{ultra-reliable low-latency communications}

==> tikz/table_tmp.tex <==
\begin{table}[t]
    \centering
    \caption{Simulation parameters ($\nu$ is the speed of light) \fs{FS: need to put on different columns to save space.}.}
    \footnotesize
    \begin{tabular}{lcc}
    \toprule
    Parameter & Symbol & Value \\ \midrule
    \multicolumn{3}{c}{\textbf{Scenario}}  \\ \midrule
    Scenario side & $D$ & $20$~m\\     
    BS position & $\mb{x}_b$ & $(25, 5, 5)\T$~m\\
    RIS element spacing & $d$ & $\nu / f_d / 2$\\
    Number of RIS elements & $N$ & 100\\
    \midrule
     \multicolumn{3}{c}{\textbf{Communication}}\\ \midrule     
     \gls{dc} frequency & $f_d$ & 3 GHz\\
     Bandwidth of \gls{dc} & $B_d$ & $180$~kHz\\  
     \gls{ue} and \gls{bs} transmit powers & $\rho_u$, $\rho_b$ & 24, 40~dBm \\     
     \gls{ue}, \gls{ris}, and \gls{bs} noise power & $\sigma_u^2, \sigma_r^2, \sigma_b^2$ & $-94$~dBm\\
     \midrule
     \multicolumn{3}{c}{\textbf{Paradigms}} \\ 
     \midrule     
     Codebooks cardinality & $C\oce$, $C\bsw^\mathrm{fix}$, $C\bsw^\mathrm{fle}$  & $N$, $\lceil N/3 \rceil$, $N$\\
     Overall frame duration & $\tau$ & [10, 200] ms \\
     \gls{tti} duration & $T$ & 0.5 ms \\
     Guard period & $\tau_s$ & 50 $\mu$s \\
     Pilot sequence length & $p$ & 1 \\
     \gls{ce} duration in \glspl{tti} & $A$ & 5 \\
     \midrule
     \multicolumn{3}{c}{\textbf{Control packet structure}} \\ \midrule
     ID bits & $b^\mathrm{ID}$ & 8\\  
     \glspl{tti} bits & $b^\mathrm{frame}$ & 16\\
     Guard period bits & $b^\mathrm{guard}$ & 16\\
     Configuration selection bits & $b^\mathrm{conf}$ & 8\\
     \gls{se} table bits & $b^\mathrm{SE}$ & 6\\
     \gls{ris} quantization level bits& $b^\mathrm{quant}$ & 2\\
     \bottomrule
    \end{tabular}
    \label{tab:params}
\end{table}
